Task-Adaptive Neural Network Search with Meta-Contrastive Learning

Most conventional Neural Architecture Search (NAS) approaches are limited in that they only generate architectures without searching for the optimal parameters. While some NAS methods handle this issue by utilizing a supernet trained on a large-scale dataset such as ImageNet, they may be suboptimal if the target tasks are highly dissimilar from the dataset the supernet is trained on. To address such limitations, we introduce a novel problem of \emph{Neural Network Search} (NNS), whose goal is to search for the optimal pretrained network for a novel dataset and constraints (e.g. number of parameters), from a model zoo. Then, we propose a novel framework to tackle the problem, namely \emph{Task-Adaptive Neural Network Search} (TANS). Given a model-zoo that consists of network pretrained on diverse datasets, we use a novel amortized meta-learning framework to learn a cross-modal latent space with contrastive loss, to maximize the similarity between a dataset and a high-performing network on it, and minimize the similarity between irrelevant dataset-network pairs. We validate the effectiveness and efficiency of our method on ten real-world datasets, against existing NAS/AutoML baselines. The results show that our method instantly retrieves networks that outperform models obtained with the baselines with significantly fewer training steps to reach the target performance, thus minimizing the total cost of obtaining a task-optimal network. Our code and the model-zoo are available at https://github.com/wyjeong/TANS.

==> algo/algo_model_zoo.tex <==
\begin{wrapfigure}{r}{0.47\textwidth}
    \vspace{-0.77in}
    \small
    \begin{algorithm}[H]
%        \begin{spacing}{0.8}
%        \SetAlgoLined
%        \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
%        \SetKwRepeat{Repeat}{repeat}{until}
%        \SetInd{0.15em}{0.8em}
%            %\Input{
%            %    $\bm D = \lbrace D_1, \dots, D_{N_D} \rbrace$: set of available datasets, $\bm M = \lbrace M_1, \dots, M_{N_M} \rbrace$: set of available architectures, $\bm Z \subset \bm D \times \bm M$: ordered set of $N_{init}$ randomly picked initial dataset-architecture pairs, $A \subset [0, 1]^{N_{init}}$: evaluated accuracies of the initial pairs $\bm Z$.
%            %}
%            
%            \While{termination condition is not met}{
%                Train accuracy predictor $f$ on data $(\bm Z, \bm A)$\;
%                Choose $\bm C \subset (\bm D \times \bm A) \setminus \bm Z$; Sample $\lbrace\alpha_i^{(j)}\rbrace_{j=1}^{N_s}$ from $p_f(\cdot | D_i, A_i)$ for each $(D_i, A_i) \in \bm C$\;
%                $\bm Z' \leftarrow \lbrace \rbrace$; $\bm{\hat{A}}' \leftarrow \lbrace \rbrace$\;%\tcc*[r]{Selected pairs and their expected accuracies}
%                \For{$k = 1 \dots N_r$} {
%                    %\For{each $(D_i, A_i) \in \bm C$} {  
%                        %$s_i \leftarrow \frac{1}{N_s}\sum_{j=1}^{N_s} \left[g_{D_i}(\bm Z' \cup \lbrace (D_i, A_i) \rbrace, \bm A' \cup \lbrace \alpha_i^{(j)} \rbrace) - g_{D_i}(\bm Z', \bm A')\right]$ for each $(D_i, A_i) \in \bm C$ where $\bm Z' = \bm Z \cup \bm Z'$, $\bm A' = \bm A\cup \bm{\hat{A}}'$ %\tcc*[r]{Estimate score for $i$-th candidate}
%                    %}
%                    $i^* \leftarrow \argmax_i S(C_i; \bm Z \cup \bm Z', \bm A \cup \bm{\hat{A}}')$\;
%                    %\tcc*[r]{Index of the expected best candidate pair}
%                    $\bm Z' \leftarrow \bm Z' \cup \lbrace C_{i^*}\rbrace$\;
%                    $\bm{\hat{A}}' \leftarrow \bm{\hat{A}}' \cup \lbrace \frac{1}{N_s} \sum_{j=1}^{N_s} \alpha_{i^*}^{(j)} \rbrace$\;
%                }
%                $\bm A' \leftarrow$ Evaluate the accuracies of $\bm Z'$\; 
%                $\bm Z \leftarrow \bm Z \cup \bm Z'$; $\bm A \leftarrow \bm A \cup \bm A'$\; 
%            }
%            \Output{Efficiently constructed model zoo $(\bm Z, \bm A)$.}
%            
%        
%            \caption{Model Zoo Construction}
%            \label{alg:modelzoo}
%        \end{spacing}
%
        \begin{spacing}{0.8}
        \SetAlgoLined
        \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
        \SetKwRepeat{Repeat}{repeat}{until}
        \SetInd{0.15em}{0.8em}
            \textbf{Input:} $\bm D, \bm M$: collection of datasets and models,\\
            \quad $\bm Z \subset \bm D \times \bm M$: $N_{init}$ initial pairs,\\
            \quad $\bm A$: accuracies of the initial pairs $\bm Z$.
            
            \While{termination condition is not met}{
                Train accuracy predictor $f$ on data $(\bm Z, \bm A)$\;
                Choose the candidate set of pairs $\bm C$\;
                $i^* \leftarrow \argmax_i \text{Score}_f(C_i; \bm Z, \bm A)$\;
                $\alpha_{i^*} \leftarrow$ Evaluate the actual accuracy of $C_{i^*}$\; 
                Append $\bm C_{i^*}$ and $\alpha_{i^*}$ to $\bm Z$ and $\bm A$\;
            }
            \Output{Efficiently constructed model zoo $(\bm Z, \bm A)$.}
            
        
            \caption{\footnotesize Model Zoo Construction ($N_r=1$)}
            \label{alg:modelzoo}
        \end{spacing}
        
    \end{algorithm}
    \vspace{-0.2in}
\end{wrapfigure} 


==> defs.tex <==

%\usepackage[numbers, sort&compress]{natbib}


\usepackage{amsmath, amssymb, bm, amsthm}
\usepackage{mathrsfs} 
\usepackage{mathtools}
\usepackage{thmtools}
\usepackage{enumitem}
\usepackage{subfigure}
\usepackage{color}
\usepackage{booktabs}
\usepackage{array}
\usepackage{tabularx, booktabs, multirow}
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}

%\usepackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}


\usepackage[capitalize,nameinlink]{cleveref}


%\numberwithin{equation}{section}
%\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
%\newtheorem{defn}{Definition}[section]
\newtheorem{lem}{Lemma}[section]
%\newtheorem{cor}{Corollary}[section]
\newtheorem{cor}{Corollary}
%\newtheorem{prop}{Proposition}[section]
%\theoremstyle{definition}
%\newtheorem{algorithm}{Algorithm}[section]
%\newtheorem{example}{Example}[section]


\newcommand{\dee}{\mathrm{d}}
\newcommand{\grad}{\nabla}

\DeclareMathOperator{\ber}{Ber}
\DeclareMathOperator{\gammadist}{Gamma}
\DeclareMathOperator{\betadist}{Beta}
\DeclareMathOperator{\dir}{Dir}
%\DeclareMathOperator{\cat}{cat}
\DeclareMathOperator{\expon}{expon}
%\DeclareMathOperator{\unif}{unif}
%\DeclareMathOperator{\KL}{KL}
\DeclareMathOperator{\sgm}{sgm}
\DeclareMathOperator{\frob}{{F}}
\DeclareMathOperator{\softmax}{{softmax}}
\DeclareMathOperator{\var}{{Var}}
\DeclareMathOperator{\diag}{{diag}}
\DeclareMathOperator{\softplus}{{Softplus}}
\DeclareMathOperator{\pool}{{StatisticsPooling}}

\newcommand{\normal}{\mathcal{N}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\card}[1]{\vert {#1} \vert}
\newcommand{\distiid}{\overset{iid}{\dist}}
\newcommand{\distind}{\overset{ind}{\dist}}
\newcommand{\Indicator}[1]{\mathds{1}_{\{#1\}}}
\newcommand{\II}{\mathbb{I}}
\newcommand{\defas}{\vcentcolon=}  % requires mathtools package
\newcommand{\iid}{i.i.d.}

\newcommand{\bepsilon}{{\boldsymbol{\epsilon}}}
\newcommand{\btheta}{{\boldsymbol{\theta}}}
\newcommand{\bTheta}{{\boldsymbol{\Theta}}}
\newcommand{\bbeta}{{\boldsymbol{\beta}}}
%%\newcommand{\E}{{\mathbb{E}}}
\newcommand{\Real}{{\mathbb{R}}}
\newcommand{\calP}{{\mathcal{P}}}
\newtheorem{observation}{Observation}

\newcommand{\bzero}{\mathbf{0}}
\newcommand{\bone}{\mathbf{1}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bof}{\mathbf{f}}
\newcommand{\bhy}{\widehat{\by}}
%\newcommand{\bW}{\mathbf{W}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\be}{\mathbf{e}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bh}{\mathbf{h}}
\newcommand{\bhW}{{\widehat{\bW}}}
\newcommand{\btW}{{\widetilde{\bW}}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bphi}{{\boldsymbol{\phi}}}
\newcommand{\bpi}{{\boldsymbol{\pi}}}
\newcommand{\noise}{{\boldsymbol{\varepsilon}}}

\newcommand{\ts}{{\tau}}

\newcommand{\bee}{\begin{eqnarray}}
\newcommand{\eee}{\end{eqnarray}}



==> figures/figure_convergence_plot.tex <==

\begin{figure}[t!]
\centering
\includegraphics[width=\linewidth]{figures/images/fig_5.eps}
\vspace{-0.2in}
\caption{\small \textbf{Comparison between Our Method and Conventional NAS Approaches}: We visualize first 10 epoch accuracy curves on unseen meta-test datasets corresponding to the Table~\ref{tbl:unseen_task}.  }
\label{fig:convergence_plot}
\end{figure}


==> figures/figure_dataset_distribution.tex <==
\begin{figure}[t!]
\centering
%\vspace{0.05in}
\includegraphics[width=\linewidth]{figures/images/latent_space_fake.png}
\caption{Dataset Distribution }%of the generator over various datasets. Each marker indicates $\bz$ of the sampled subset of each dataset with different seed.} 
\label{fig:dataset_distribution}
\end{figure}
%\vspace{-0.2in}

==> figures/figure_model_zoo_cons.tex <==
\begin{figure}[t!]
\centering
%\vspace{0.05in}
\includegraphics[width=\linewidth]{figures/images/model_zoo_cons.png}
\caption{Comparison of Uncertainty-Aware Search to Random Search}
\label{fig:modelzoocons}
\end{figure}
%\vspace{-0.2in}

==> figures/figure_predictor.tex <==
\begin{figure}[t]
% \vspace{-0.1in}
\centering
% \includegraphics[width=0.95\linewidth]{figures/images/latent_space.pdf}
% \includegraphics[width=0.85\linewidth]{figures/images/fig_pred.pdf}

\begin{tabular}{c c c}
    
    \includegraphics[width=0.33\linewidth]{figures/images/latent_space.pdf}
    &  \includegraphics[width=0.33\linewidth]{figures/images/model_zoo.pdf}
    & \includesvg[width=0.2\linewidth]{figures/images/3d}
    \\
    
    \small (a) Model-Zoo Visualization
    &  \small (b) Number of Trained Networks
    &  \small (c) Pareto Optimal Curve
    
\end{tabular}


\caption{\small \blu{\textbf{Analysis of Model-Zoo Construction}: (a) we visualize the latent representation of datasets and networks with their accuracy on the cross-modal latent space using T-SNE. Abbreviated TRAF and UCF denotes the Traffic Signs and UCF-AI datasets. (b) we compare performance between our model-zoo with smaller number of networks (ours is 14,000). (c) our model zoo is constructed with Pareto-efficient pairs}}
\label{fig:latent_space_and_pred}
\vspace{-0.2in}
\end{figure}


==> figures/figure_recall.tex <==
\begin{figure}[t!]
\centering
%\vspace{0.05in}
\includegraphics[width=\linewidth]{figures/images/ep_1000.png}
\vspace{-0.3in}
\caption{\textbf{R@1 Scores over Training Epochs:} We visualize R@1 curves during training until $1,000$ training epochs while varying our model components corresponding to the Table~\ref{tbl:retrieval}.} 
\label{fig:recall_curve}
\end{figure}
%\vspace{-0.2in}

==> figures/figure_test_dataset.tex <==
\begin{figure*}[!t]
\centering
\caption{
\textbf{Example of Unseen Query Datasets}. 
}

\includegraphics[width=.24\columnwidth]{figures/images/tmp.png}
\includegraphics[width=.24\columnwidth]{figures/images/tmp.png}
\includegraphics[width=.24\columnwidth]{figures/images/tmp2.png}
\includegraphics[width=.24\columnwidth]{figures/images/tmp2.png}
\includegraphics[width=.24\columnwidth]{figures/images/tmp.png}
\includegraphics[width=.24\columnwidth]{figures/images/tmp.png}
\includegraphics[width=.24\columnwidth]{figures/images/tmp2.png}
\includegraphics[width=.24\columnwidth]{figures/images/tmp2.png}
\label{fig:unseen_query_dataset}
\end{figure*}

==> figures/wrap_fig_model_zoo_viz.tex <==
\includegraphics[width=0.5\linewidth]{figures/images/latent_space.pdf}

==> figures/wrap_fig_perf_pred.tex <==
\begin{wrapfigure}[10]{r}{5.5cm}
    \vspace{-0.3in}
    \begin{center}
        \includegraphics[width=0.4\columnwidth]{figures/images/fig_pred.pdf}
    \end{center}
    \vspace{-0.175in}
    \caption{\small Performance Gain }
    \label{fig:perf_pred}
\end{wrapfigure}

==> figures/wrap_retrived_arch.tex <==
\begin{wrapfigure}[9]{r}{0.3\textwidth}
    \vspace{-0.35in}
    \begin{center}
        \includegraphics[width=0.3\textwidth]{figures/images/retrieved_neural_arch.pdf}
    \end{center}
    \vspace{-0.175in}
    \caption{\small Gain by Architecture}
    \label{fig:arch}
\end{wrapfigure}

==> tables/arch_meta_test.tex <==
\begin{wraptable}[8]{r}{4.25cm}
    \vspace{-0.15in}
    \centering
    \caption{\small Effects of Topology}
    \vspace{-0.05in}
    \resizebox{0.3\columnwidth}{!}{
        \vspace{-0.2in}
            \begin{tabular}{l|c}
                \toprule
                    Model & 
                    Averaged Acc.\\
                    \midrule 
                    \midrule
                    FBNet-A~\citep{wu2019fbnet}  &  93.00\small{$\pm$1.95}    \\
                    OFA~\citep{cai2020once}      &  93.89\small{$\pm$0.84}    \\
                    MetaD2A~\citep{lee2021rapid} &  95.24\small{$\pm$1.14}    \\
                    \midrule
                    TANS w/o Topol.              &  95.24\small{$\pm$0.21}    \\
                    TANS (Ours)                         &  \textbf{96.28\small{$\pm$0.30}}    \\
                 \bottomrule
                \end{tabular}
                \label{tbl:abl}
        }
    \vspace{-0.1in}
    \label{tbl:wo_topol}
\end{wraptable}

==> tables/predictor_mse.tex <==
\begin{table}[]
    \begin{center}
        \begin{tabular}{l|cccc}
        \toprule
        \centering
        Model             & \# of Samples & Wall clock time & Latency & Accuracy \\
        \midrule
        MobileNetV2       & x             & x               & x       & x        \\
        NASNet-A          & x             & x               & x       & x        \\
        DARTS             & x             & x               & x       & x        \\
        MnasNet           & x             & x               & x       & x        \\
        FBNet-C           & x             & x               & x       & x        \\
        ProxylessNAS      & x             & x               & x       & x        \\
        MobileNetV3-Large & x             & x               & x       & x        \\ 
        OFA               & x             & x               & x       & x        \\
        \midrule
        OFA +Ours         & x             & x               & x       & x        \\ 
        \bottomrule
        \end{tabular}
    \end{center}
\end{table}

==> tables/retrieval_abl.tex <==
% \begin{figure*}[t!]
%     \vspace{-0.125in}
%     \begin{minipage}{0.49\linewidth}
%         \centering
%         \small
%         \vspace{-0.05in}
%         \captionof{table}{\small \textbf{Evaluation of the retrieval performance.} We evaluate the retrieval performance for \textit{unseen instances} (from a validation set) as a query, on our model zoo containing \textbf{\textit{14,000}} trained models, with different learning strategies, such as cosine similarity (Cosine), hard negative loss (Hard Neg.) that considers one maximum negative instance, or contrastive loss (Contrastive) that considers all negative instances, compared with the random and largest parameter selection baselines for architecture selection.}
%         \vspace{-0.11in}
%     	\begin{center}
%          \resizebox{1.0\linewidth}{!}{
%             \begin{tabular}{lccccc}
%             \toprule
%                 \multicolumn{1}{c}{\multirow{2}{*}{Model}} & 
%                 \multicolumn{5}{c}{Performance of The Same Pair Retrieval}\\
%                                   &      
%                 R@1 & R@5 & R@10 & Mean & Median \\
%                 \midrule 
%                 \midrule
%                 Random &
%                 2.14           & 
%                 2.86           & 
%                 8.57           & 
%                 69.04           & 
%                 70.0          \\
%                 Largest Parameter &
%                 3.57           & 
%                 7.14           & 
%                 10.00           & 
%                 51.85           & 
%                 52.0           \\
%                  \midrule
%                  TANS + Cosine & % (Ours)
%                     9.29 & 12.86 &	22.14 & 46.02	& 38.0 \\ %& 8642
%                 %   29.3                 & 
%                 %   50.0                 & 
%                 %   56.4                 & 
%                 %   25.4                 & 
%                 %   5.0                  \\
%                 TANS + Hard Neg. & % (Ours)
%                   72.14 & 84.29 & 88.57 & 4.86 & 1.0 \\ %&9553 
%                  \textbf{TANS + Contrastive}  &  %(Ours) 
%                  \textbf{80.71}                  & 
%                  \textbf{96.43}                  & 
%                  \textbf{99.29}                  & 
%                  \textbf{1.90}                   & 
%                  \textbf{1.0}                   \\ 
%                 %  \textbf{9564}\\
%                 \midrule
%                 TANS w/o Predictor & 
%                     80.00 &	\textbf{96.43} & 97.86 & 2.23 &	\textbf{1.0}  \\ %9517

%              \bottomrule
%             \end{tabular}
%     	    }
%     	\end{center}
%         \small
%         \label{tbl:retrieval-abl-loss}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{0.49\linewidth}
        
        
%     \end{minipage}
%     \vskip -0.125in
% \end{figure*}


% \captionof{table}{\small \textbf{Ablation study of TANS on the retrieval task.} We perform the retrievals as in the Table~\ref{tbl:retrieval-abl-loss}, while varying the model embedding methods among, Graph Isomorphism Network (GIN), Variational Autoencoder for Directed Acyclic Graphs (D-VAE), and using auxiliary information about the topology as suggested by Once-For-All (OFA). We also ablate the proposed model by deleting a key component of it at a time, such as the performance predictor (Predictor) or the functional embedding (Func.Emb.).}
%         \vspace{-0.125in}
%     	\begin{center}
%          \resizebox{1.0\linewidth}{!}{
%             \renewcommand{\arraystretch}{0.95}
%             \begin{tabular}{lccccc}
%             \toprule
%                 \multicolumn{1}{c}{\multirow{2}{*}{Model}} & 
%                 \multicolumn{5}{c}{Performance of The Correct Pair Retrieval}\\
%                                   &      
%                 R@1 & R@5 & R@10 & Mean & Median \\ % & Ep@Max 
%                 \midrule 
%                 \midrule
%                 \textbf{TANS (Ours)} &
%                     \textbf{80.71}               & 
%                     \textbf{96.43}                      & 
%                     \textbf{99.29}                & 
%                     \textbf{1.90}                & 
%                     \textbf{1.0}                  
%                     \\ %9564
%                 \midrule
%                  TANS w/ GIN                 &
%                     76.43		          & 
%                     93.57                & 
%                     96.43               & 
%                     2.58	              & 
%                     \textbf{1.0}                  
%                     \\ % 9874
                    
%                 TANS w/ D-VAE & 
%                     80.00              & 
%                     95.71                & 
%                     97.14                 & 
%                     1.92                 & 
%                     \textbf{1.0}                  
%                     \\ %8205
%                 \midrule
%                 TANS w/o Predictor & 
%                     80.00 &	\textbf{96.43} & 97.86 & 2.23 &	\textbf{1.0}  \\ %9517
                    
%                 TANS w/o Func.Emb. &
%                     5.00	& 11.43	& 18.57 & 63.20	& 63.0	\\ %6913
%              \bottomrule
%             \end{tabular}
%     	    }
%     	\end{center}
%         \small
%         \label{tbl:retrieval}


==> tables/retrieval_abl_component.tex <==
\begin{table*}[t!]
	\caption{\small \textbf{NAS Results on Average of 9 Unseen Devices (Meta-Test)} }%MetaD2A conducts amortized inference on unseen target datasets after meta-training on source database consisting of subsets of ImageNet-1K and architectures of NAS-Bench-201 search space. Meta-training time is 12.7/8.4 GPU hours for the generator/the predictor. For fair comparison, the parameters of searched architectures are trained on each dataset from scratch instead of transferring parameters from ImageNet. $T$ is the time to construct precomputed architecture database for each target. We report accuracies with $95\%$ confidence intervals. } %  45797/30152 GPU seconds
	\vspace{-0.15in}
	\small
	\begin{center}
     \resizebox{\linewidth}{!}{
	    \begin{tabular}{cl|ccccc}
	   	\toprule
	   	\multirow{2}{*}{Search Space}                   & 
	   	\multicolumn{1}{c|}{\multirow{2}{*}{NAS Method}} & 
	   	\# of Samples                               & 
	   	Build Time                                  & 
	   	\multirow{2}{*}{Speed Up}                   &
    	Latency                                     & 
	   	Accuracy                                    \\ 
	   	                                            & 
	   	                                            & 
	   	(N)                                         & 
	   	(Sec)                                       & 
	   	                                            & 
        (ms)                                        & 
	   	(\%)                                        \\
	   	\midrule
	   	\midrule
%%%%%%%%%%%%%%%%%%%%%%%%   MobileNetV3  %%%%%%%%%%%%%%%%%%%%%%%%%
	   	\multirow{2}{*}{MobileNetV3}               &%~\citep{howard2019searching}                 &
	    OFA~\citep{cai2020once}                    &
	   	xxx                                        &
	   	xxxx                                       &
	    xxx$\times$                                &
	    x.xx	   		   	                       &
	   	x.xx\tiny$\pm$x.xx                        \\	   	
	   	                                           &
	   	\textbf{Ours}                              &
	   	\textbf{xx}                                &
	   	\textbf{xx}                                &
	   	x$\times$                                  &
	   	\textbf{x.xxx}	   		   	               &
	   	\textbf{xx.xx\tiny$\pm$x.xx}               \\
	   	\midrule
%%%%%%%%%%%%%%%%%%%%%%%%   Nas-Bench-201  %%%%%%%%%%%%%%%%%%%%%%%%%
	   	\multirow{2}{*}{NAS-Bench-201}             &%~\citep{howard2019searching}                 &
	    MetaD2A~\citep{lee2021rapid}               &
	   	xxx                                        &
	   	xxxx                                       &
	    xxx$\times$                                &
	    x.xx	   		   	                       &
	   	x.xx\tiny$\pm$x.xx                        \\	   	 	
	   	                                           &
	   	\textbf{Ours}                              &
	   	\textbf{xx}                                &
	   	\textbf{xx}                                &
	   	x$\times$                                  &
	   	\textbf{x.xxx}	   		   	               &
	   	\textbf{xx.xx\tiny$\pm$x.xx}               \\
	   	\midrule
%%%%%%%%%%%%%%%%%%%%%%%%   HAT  %%%%%%%%%%%%%%%%%%%%%%%%%
	   	\multirow{2}{*}{HAT (NLP)}             &%~\citep{howard2019searching}                 &
	    HAT~\cite{wang2020hat}                     &
	   	xxx                                        &
	   	xxxx                                      &
	    xxx$\times$                                &
	    x.xx	   		   	                       &
	   	x.xx\tiny$\pm$x.xx                        \\	   	  	
	   	                                           &
	   	\textbf{Ours}                              &
	   	\textbf{xx}                                &
	   	\textbf{xx}                                &
	   	x$\times$                                  &
	   	\textbf{x.xxx}	   		   	               &
	   	\textbf{xx.xx\tiny$\pm$x.xx}               \\
	   	\bottomrule
        \end{tabular}
	    }
	\end{center}
	\small
	\label{tbl:nas}
	\vspace{-0.15in}
	
\end{table*}

==> tables/retrieval_abl_wrap.tex <==

\begin{wraptable}[9]{r}{6.5cm}
    \vspace{-0.225in}
    \centering
    \small 
    \caption{Analysis of Retrieval Performance}
    \vspace{-0.05in}
    \resizebox{0.475\columnwidth}{!}{
        \vspace{-0.2in}
            \begin{tabular}{lccccc}
                \toprule
                    \multicolumn{1}{c}{\multirow{2}{*}{Model}} & 
                    \multicolumn{5}{c}{Performance of The Same Pair Retrieval}\\
                                      &      
                    R@1 & R@5 & R@10 & Mean & Median \\
                    \midrule 
                    \midrule
                    Random &
                    2.14           & 
                    2.86           & 
                    8.57           & 
                    69.04           & 
                    70.0          \\
                    Largest Parameter &
                    3.57           & 
                    7.14           & 
                    10.00           & 
                    51.85           & 
                    52.0           \\
                     \midrule
                     TANS + Cosine & % (Ours)
                        9.29 & 12.86 &	22.14 & 46.02	& 38.0 \\ %& 8642
                    %   29.3                 & 
                    %   50.0                 & 
                    %   56.4                 & 
                    %   25.4                 & 
                    %   5.0                  \\
                    TANS + Hard Neg. & % (Ours)
                       72.14 & 84.29 & 88.57 & 4.86 & 1.0 \\ %&9553 
                     \textbf{TANS + Contrastive}  &  %(Ours) 
                     \textbf{80.71}                  & 
                     \textbf{96.43}                  & 
                     \textbf{99.29}                  & 
                     \textbf{1.90}                   & 
                     \textbf{1.0}                   \\ 
                    %  \textbf{9564}\\
                    \midrule
                    TANS w/o Func.Emb. & 
                        5.00 &	11,43 & 18.57 & 63.20 &	63.0  \\
                    TANS w/o Predictor & 
                        80.00 &	\textbf{96.43} & 97.86 & 2.23 &	\textbf{1.0}  \\ %9517
                    
                 \bottomrule
                \end{tabular}
                \label{tbl:arch_meta_test}
        }
    \vspace{-0.1in}
\end{wraptable}


==> tables/tbl_automl.tex <==

\begin{wraptable}{r}{5.5cm}
    \vspace{-0.2in}
    \centering
    \small{\caption{\small w/ AutoML Platforms}} 
    \vspace{-0.05in}
    \resizebox{0.4\columnwidth}{!}{
            \vspace{-0.2in}
            \begin{tabular}{lcc}
	   	\toprule
	   	
	   	\multicolumn{1}{c}{\multirow{2}{*}{Method}}                  & 
	   %	Params                                                       &
	   	Total Times                                                  &
	   	Accuracy                                                    \\
	   	
	   	
	   %	&(M)
	   	&(GPU sec)&(\%)\\
	   	
	   	\midrule
	   	\midrule
        Custom Vision                                     &
        % x.xx                                              &
        3600                           &
        96.15\tiny$\pm$2.52                              \\
                       
	    Vision Edge                                     &
        % x.xx                                            &
        4608                            &
        97.05\tiny$\pm$0.85                             \\
                 
	   	                                           
        % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        % \cdashline{1-4}\noalign{\vskip 0.75ex}
        % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	   	\midrule                             
	   	
	   	\textbf{TANS (Ours) }                           & 
	   %	5.51                                            &
	   	\textbf{209} & %.95$\pm$11.01                    &
	   	\textbf{98.11\tiny$\pm$0.30}                    \\       
	   	
	   	\bottomrule
	   	
	   	\end{tabular}
    }
    \vspace{-0.1in}
\end{wraptable}




==> tables/tbl_modelzoo.tex <==


\begin{wraptable}[5]{r}{5cm}
    \vspace{-0.25in}
    \small
    \caption{Search \& Pretraining Costs }
    \vspace{-0.05in}
    \resizebox{0.35\textwidth}{!}{
        \begin{tabular}{l|c|c}
    	   \toprule 
    	   \centering
    	   \multirow{2}{*}{Method}                 & 
    	   Architecture                            &
    	   Retrieved Dataset                       \\
    	   &
    	   Search Cost                             &
    	   Pre-training Cost                       \\
          \midrule
          \midrule
          Conventional NAS                         & 
          O(N)                                     &
          O(N)                                     \\
          MetaD2A                                  & 
          O(1)                                     &
          O(N)                                     \\
          \textbf{TANS (Ours)}                     &
          \textbf{O(1)}                            &
          \textbf{O(1)}                            \\
    	  \bottomrule
       \end{tabular} 		
    }
    \label{tbl:cost}
\vspace{-0.1in}
\end{wraptable}

